AdaptDiff: Cross-Modality Domain Adaptation via Weak Conditional Semantic Diffusion for Retinal Vessel Segmentation

Deep learning has shown remarkable performance in medical image segmentation. However, despite its promise, deep learning has many challenges in practice due to its inability to effectively transition to unseen domains, caused by the inherent data distribution shift and the lack of manual annotations to guide domain adaptation. To tackle this problem, we present an unsupervised domain adaptation (UDA) method named AdaptDiff that enables a retinal vessel segmentation network trained on fundus photography (FP) to produce satisfactory results on unseen modalities (e.g., OCT-A) without any manual labels. For all our target domains, we first adopt a segmentation model trained on the source domain to create pseudo-labels. With these pseudo-labels, we train a conditional semantic diffusion probabilistic model to represent the target domain distribution. Experimentally, we show that even with low quality pseudo-labels, the diffusion model can still capture the conditional semantic information. Subsequently, we sample on the target domain with binary vessel masks from the source domain to get paired data, i.e., target domain synthetic images conditioned on the binary vessel map. Finally, we fine-tune the pre-trained segmentation network using the synthetic paired data to mitigate the domain gap. We assess the effectiveness of AdaptDiff on seven publicly available datasets across three distinct modalities. Our results demonstrate a significant improvement in segmentation performance across all unseen datasets. Our code is publicly available at https://github.com/DeweiHu/AdaptDiff.

==> tables/qualitative_table.tex <==
\setlength{\tabcolsep}{1pt}
\begin{figure}[t]
    \centering
    \begin{tabular}{cccccc}
         & $\mathbf{x}^\mathcal{S}$ & $\mathbf{y}$ & {\scriptsize \textbf{CycleGAN}} & {\scriptsize \textbf{SynSeg}} & {\scriptsize \textbf{AdaptDiff}} \\
         
         \rotatebox{90}{\hspace{0.2cm} \scriptsize \textbf{OCTA-500}} & 
         \includegraphics[width=0.185\linewidth]{imgs/img_1.png} &
         \includegraphics[width=0.185\linewidth]{imgs/mask_1.png} &
         \includegraphics[width=0.185\linewidth]{imgs/cyclegan_1.png} &
         \includegraphics[width=0.185\linewidth]{imgs/synseg_1.png} &
         \includegraphics[width=0.185\linewidth]{imgs/diff_1.png} \\

        \rotatebox{90}{\hspace{0.6cm} \scriptsize \textbf{ROSE}} & 
         \includegraphics[width=0.185\linewidth]{imgs/img_3.png} &
         \includegraphics[width=0.185\linewidth]{imgs/mask_3_marked.jpg} &
         \includegraphics[width=0.185\linewidth]{imgs/cyclegan_3_marked.jpg} &
         \includegraphics[width=0.185\linewidth]{imgs/synseg_3_marked.jpg} &
         \includegraphics[width=0.185\linewidth]{imgs/diff_3_marked.jpg} \\
        
         \rotatebox{90}{\hspace{0.4cm} \scriptsize \textbf{PRIME}} & 
         \includegraphics[width=0.185\linewidth]{imgs/img_2.png} &
         \includegraphics[width=0.185\linewidth]{imgs/mask_2_marked.jpg} &
         \includegraphics[width=0.185\linewidth]{imgs/cyclegan_2_marked.jpg} &
         \includegraphics[width=0.185\linewidth]{imgs/synseg_2_marked.jpg} &
         \includegraphics[width=0.185\linewidth]{imgs/diff_2_marked.jpg} \\
         
    \end{tabular}
    \caption{Synthetic images from  the image alignment approaches. The yellow boxes  highlight  spurious vessels, red boxes highlight missing vessels, for CycleGAN and SynSeg outputs. AdaptDiff-synthesized images have the correct anatomy in both areas.}
    \label{fig:qualitative1}
\end{figure}

==> tables/table2.tex <==
\renewcommand{\arraystretch}{0.95}
\begin{table}[t]
    \centering
    \begin{tabular}{p{0.15\textwidth}>{\centering}
                    p{0.2\textwidth}>{\centering\arraybackslash}
                    p{0.2\textwidth}>{\centering\arraybackslash}
                    p{0.2\textwidth}>{\centering\arraybackslash}
                    p{0.2\textwidth}}
        \specialrule{.1em}{.05em}{.05em}
        
        \hspace{0.1em} {\scriptsize Method} & {\scriptsize OCTA 500(3M)} & {\scriptsize OCTA 500(6M)} & {\scriptsize ROSE} & {\hspace{-0.2em}\scriptsize RECOVERY}\\
         
        \specialrule{.1em}{.05em}{.05em}
        \scriptsize \hspace{0.08em} \textit{baseline} & $\scalemath{0.9}{65.97 \pm 7.56}$ & $\scalemath{0.9}{73.16 \pm 4.54}$ & $\scalemath{0.9}{67.41 \pm 3.35}$ & $\scalemath{0.9}{60.98 \pm 4.20}$ \\
        \hline
        \scriptsize \hspace{0.3em} DANN \cite{javanmardi2018domain} & $\scalemath{0.9}{69.27 \pm 9.81}$ & $\scalemath{0.9}{80.93 \pm 3.31}$ & $\scalemath{0.9}{70.37 \pm 8.21}$ & $\scalemath{0.9}{66.33 \pm 3.77}$ \\
        \scriptsize CycleGAN \cite{palladino2020unsupervised} & $\scalemath{0.9}{31.97 \pm 3.90}$ & $\scalemath{0.9}{37.47 \pm 3.13}$ & $\scalemath{0.9}{16.05 \pm 2.31}$ & $\scalemath{0.9}{22.95 \pm 2.41}$ \\
        \scriptsize \hspace{0.25em} SynSeg \cite{huo2018synseg} & $\scalemath{0.9}{44.15 \pm 3.86}$ & $\scalemath{0.9}{47.99 \pm 3.29}$ & $\scalemath{0.9}{42.42 \pm 3.09}$ & $\scalemath{0.9}{36.68 \pm 2.57}$ \\
        \scriptsize \hspace{0.15em} Proposed & $\scalemath{0.9}{\bf{72.73 \pm 5.34}}^{\dagger}$ & $\scalemath{0.9}{\bf{81.94 \pm 2.76}}^{\dagger}$ & $\scalemath{0.9}{\bf{76.15 \pm 2.55}}^{\dagger}$ & $\scalemath{0.9}{\bf{71.38 \pm 2.72}}^{\dagger}$ \\
        \hline
        \scriptsize \hspace{0.5em} \textit{oracle} & $\scalemath{0.9}{87.61 \pm 2.13}$ & $\scalemath{0.9}{84.78 \pm 2.79}$ & $\scalemath{0.9}{78.74 \pm 2.47}$ & $\scalemath{0.9}{77.13 \pm 2.72}$ \\
        \specialrule{.1em}{.05em}{.05em}
    \end{tabular}
    \caption{Dice scores (\%) for testing on target domains. Boldface: best result, underline: second best result. $^\dagger: \text{p-value} \ll 0.05$ in paired t-test compared to the baseline.}
    \label{tab:result}
\end{table}
